Learning Log-Determinant Divergences for Positive Definite Matrices

Representations in the form of Symmetric Positive Definite (SPD) matrices have been popularized in a variety of visual learning applications due to their demonstrated ability to capture rich second-order statistics of visual data. There exist several similarity measures for comparing SPD matrices with documented benefits. However, selecting an appropriate measure for a given problem remains a challenge and in most cases, is the result of a trial-and-error process. In this paper, we propose to learn similarity measures in a data-driven manner. To this end, we capitalize on the \alpha\beta-log-det divergence, which is a meta-divergence parametrized by scalars \alpha and \beta, subsuming a wide family of popular information divergences on SPD matrices for distinct and discrete values of these parameters. Our key idea is to cast these parameters in a continuum and learn them from data. We systematically extend this idea to learn vector-valued parameters, thereby increasing the expressiveness of the underlying non-linear measure. We conjoin the divergence learning problem with several standard tasks in machine learning, including supervised discriminative dictionary learning and unsupervised SPD matrix clustering. We present Riemannian gradient descent schemes for optimizing our formulations efficiently, and show the usefulness of our method on eight standard computer vision tasks.

==> Ablation_Study.tex <==
\section{Ablation study}

\subsection{Evaluation of Joint Learning}
In Table~\ref{tab:paramatoms}, we evaluate the usefulness of the learning the information divergence against learning the dictionary on the Virus dataset. For this experiment, we evaluated three scenarios, (i) fixing the dictionary to the initialization (using KMeans), and learning the parameters $\alpha,\beta$ using the IDDL-S variant, (ii) fixing $\alpha,\beta$ to the initialization using GridSearch, while learning the dictionary, and (iii) learning both dictionary and the parameters jointly. As the results in Table~\ref{tab:paramatoms} shows, jointly learning the parameters demonstrates better results, thus justifying our IDDL formulation.


\begin{table}[htbp]
\centering
\begin{adjustbox}{width= 0.9\linewidth}
\renewcommand{\arraystretch}{1.2} 
\begin{tabular}{c|c|c|c}
\textbf{Atoms | Method}   & \textbf{IDDL-Fix$(\alpha,\beta)$}  & \textbf{IDDL-Fix$(\mathbf{B})$} & \textbf{IDDL-N}\\
\hline
\textbf{15} & \textbf{78.33\%}& 61.67\% & 77.33\%\\
\hline
\textbf{45} & 80.33\%& 70.00\% & \textbf{83.67\%}\\
\hline
\textbf{75} & 81.67\%& 76.00\% & \textbf{82.33\%}\\
\end{tabular}
\end{adjustbox}
\caption{Performance evaluation of IDDL on a single split of the Virus dataset when fixing the dictionary atoms against fixing the parameters, and jointly learning the atoms and the parameters.}
\label{tab:paramatoms}
\end{table}


\subsection{Trajectories of $\alpha,\beta$}
In this experiment, we demonstrate the BCD trajectories of $\alpha$ and $\beta$ for the IDDL-S and IDDL-N variants of our algorithm on the Virus dataset. Specifically, in Figure~\ref{fig:trajectory}, we show how the value of $\alpha$ and $\beta$ varies as the BCD iteration progresses. In this experiment, we used 15 dictionary atoms. All experiments used the same initializations for the invariants. We also plot the corresponding objective and training accuracies. For IDDL-N, recall that the parameters are vectors, and thus we plot the average $\alpha$ and $\beta$ respectively. We also plot for various initializations for these parameters. 

For IDDL-S, it appears that different initializations leads to disparate points of convergence. However, for all points of convergence, the objective convergence is very similar (and so is the training accuracy), suggesting that there are multiple local minima that leads to similar empirical results. We also find that initializing with $\alpha=1.0$ demonstrates slightly better convergence than other possibilities, which we observed for other datasets too. For IDDL-N, we found that the mean of the parameters remained more or less constant, although the exact values varied by $\pm 0.2\%$ (not shown).

\begin{figure*}[t]
\subfigure[]{\includegraphics[width=6cm,trim={0 7cm 1cm 7cm},clip]{Images/alpha_beta_virus_sab.pdf}}
\subfigure[]{\includegraphics[width=6cm,trim={0 7cm 1cm 7cm},clip]{Images/obj_virus_sab.pdf}}
\subfigure[]{\includegraphics[width=6cm,trim={0 7cm 1cm 7cm},clip]{Images/traintest_virus_sab.pdf}}\\
\subfigure[]{\includegraphics[width=6cm,trim={0 7cm 1cm 7cm},clip]{Images/alpha_beta_virus_vab.pdf}}
\subfigure[]{\includegraphics[width=6cm,trim={0 7cm 1cm 7cm},clip]{Images/obj_virus_vab.pdf}}
\subfigure[]{\includegraphics[width=6cm,trim={0 7cm 1cm 7cm},clip]{Images/traintest_virus_vab.pdf}}
\caption{(a,d) Trajectory of $\alpha$ and $\beta$ over BCD iterations on the virus dataset, (b,e) shows the respective objective descent, and (c,f) shows the training set accuracy. We plot for various initializations of $\alpha$ and $\beta$.}
\label{fig:trajectory}
\end{figure*}
